Bayesian Persuasion in Sequential Trials

We consider a Bayesian persuasion or information design problem where the sender tries to persuade the receiver to take a particular action via a sequence of signals. This we model by considering multi-phase trials with different experiments conducted based on the outcomes of prior experiments. In contrast to most of the literature, we consider the problem with constraints on signals imposed on the sender. This we achieve by fixing some of the experiments in an exogenous manner; these are called determined experiments. This modeling helps us understand real-world situations where this occurs: e.g., multi-phase drug trials where the FDA determines some of the experiments, funding of a startup by a venture capital firm, start-up acquisition by big firms where late-stage assessments are determined by the potential acquirer, multi-round job interviews where the candidates signal initially by presenting their qualifications but the rest of the screening procedures are determined by the interviewer. The non-determined experiments (signals) in the multi-phase trial are to be chosen by the sender in order to persuade the receiver best. With a binary state of the world, we start by deriving the optimal signaling policy in the only non-trivial configuration of a two-phase trial with binary-outcome experiments. We then generalize to multi-phase trials with binary-outcome experiments where the determined experiments can be placed at any chosen node in the trial tree. Here we present a dynamic programming algorithm to derive the optimal signaling policy that uses the two-phase trial solution's structural insights. We also contrast the optimal signaling policy structure with classical Bayesian persuasion strategies to highlight the impact of the signaling constraints on the sender.

==> V_Discussion.tex <==
\section{Discussion}

\subsection{Non-binary Outcome Experiments} \label{sec:nonbinaryexp}
In Section \ref{sec:multiphase}, we proposed a dynamic programming algorithm to solve the optimal signaling strategy in binary-outcome experiments. When the experiments have non-binary outcomes, the same approach still works with an increased number of phases (if complexity is not an issue). 

For example, with the tuple (Input,{Outcomes}) representing experiments, consider an experiment with 3 outcomes - $E=(I_1,\{O_1,O_2,O_3\})$. Then $E$ is equivalent to a sequence of 3 binary-outcome experiments $E_1=(I_1,\{I_2,I_3\})$, $E_2=(I_2,\{O_1,O_2\})$, and $E_3=(I_3,\{O_3,O_3\})$. Every belief evolution $p \rightarrow (p_1,p_2,p_3)$ generated via $E$ can be reproduced using $E_1$, $E_2$, and $E_3$. %Hence, given a non-binary experiment, predetermined or sender-designed, we can produce a set of equivalent binary-outcome experiments and solve for the optimal sender signaling strategy.
For general non-binary experiments, see the proof of the following claim for a detailed construction from non-binary to binary experiments.
\begin{clm}\label{clm:nbnry}
Given a non-binary experiment $E=\{q_{1,1},...,q_{1,n};q_{2,1},...,q_{2,n}\}$, we can replace it by $\lceil \log_2n \rceil$ level of binary outcome experiments.
\end{clm}
%  \begin{lem}
% In a binary state world where the experiment pair $E_a,E_b$ in trial 2 have non-binary outcomes, there is a binary-outcome experiment pair $E_a',E_b'$ where the optimal strategy and the expected utility of $E_a',E_b'$ are the same as the experiment pair $E_a,E_b$ if the following condition holds:
% \end{lem}
% %{\color{red} Need to find a better way to describe the properties in the above lemma}

% \begin{lem}
% In a binary state world where every experiment in the set of possible experiments $\{E_i\}$ in trial 2 has binary outcomes, there exists an optimal strategy where the experiment chosen in phase one is a binary-outcome experiment.
% \end{lem}

\subsection{Receiver's optimal experiments} \label{sec:receiveroptexp}
In many real-world applications, the receiver can design/determine some of the experiments ahead of time for all future senders. For example, the FDA can determine regulations (the experiments) ahead of time for future trials. In such scenarios, the receiver aims to design the experiments to maximize her expected utility by circumscribing the sender's ability to tailor the interim beliefs. However, while determining the experiments, we assume that the receiver has no information about the prior in each future case or has minimal information about the prior in future cases. In such scenarios, by viewing the future prior (distribution) as a choice made by nature, the receiver now faces uncertainty on nature's strategy. This problem falls into the problem category of picking the decision rule under subjective/non-additive expected utilities with this interpretation. Assuming the axiom of uncertainty aversion, maximin strategies that were axiomatized by Gilboa and Schmeidler \cite{GILBOA1989141}, are favored in when neither the degree of the uncertainty nor agents' uncertainty aversion level is negligible. In the rest of this discussion, we assume that the receiver uses the maximin strategy to design/choose the optimal experiments and discuss two examples in binary-outcome two-phase trials. The first example considers the simplest case where the receiver can design both phase-II experiments but has no knowledge about the prior distribution. In this example, a straightforward result states that the receiver will force the sender to reveal truthfully. The second example considers a more complex scenario where the receiver can only design one of the two phase-II experiments. However, he knows the possible priors in future cases\footnote{Specifically, the receiver knows the support of the prior but the distribution of the prior is still unknown.}. Before presenting the examples, we pause to add that at the moment, we are unable to extend our analysis to multi-phase trials where the receiver can devise experiments in the middle phases. We believe that the results of \cite{doval2020sequential} could be useful in this context but again leave this exploration to future work.

%\textcolor{violet}{1-2 sentences should be added here to mention the receiver problem is non-trivial, related to what discussed in example 2.}
%The receiver's optimal experiments design in general multi-phase trials will be a future direction of this work.

% {\color{blue} Need to justify why the maximin is chosen by the receiver
%, e.g., "Equilibrium in Beliefs under Uncertainty," Kin Chung Lo, JET, 1996 
% "Ambiguous Games," Massimo Marinacci, GEB, 2000.
% Ellsberg paradox, Uncertainty Aversion.
% Models favor maximin strategies when players understand that they face uncertainty on their opponents' strategies.
% }

\subsubsection{Example: Receiver has full control in phase-II experiments in a two-phase trial}
    Let's use the same model analyzed in Section \ref{sec:BOE} as an example to shed some light on the receiver's optimal experiments. First, we consider the case where the receiver can control both experiments in phase II. In other words, the receiver can design parameters $q_{A1},q_{A2},q_{B1},q_{B2}$. To avoid redundant discussions and to simplify the analysis, we still assume these parameters satisfy the assumptions made in Claim \ref{clm_asp}. When there are no real-world constraints on how precise the experiments can be, i.e., $q_{A1},q_{A2},q_{B1},q_{B2}\in [0,1]$, and the receiver uses a maximin strategy among all possible priors, his optimal experiments are stated in the following lemma.
    
	\begin{lem} \label{lem:receiverexp}
	If the receiver can design phase-II experiments with no constraints, then her optimal experiments $E_A,E_B$ are $E_A=(q_{A1},q_{A2})=(1,0)$ and $E_B=(q_{B1},q_{B2})=(1,0)$. In other words, the experiment outcome will reveal the true state regardless of the prior and interim beliefs.
	\end{lem}
    %When we allow the receiver to design experiments without any constraints, the receiver will pick two revealing experiments in phase-II to guarantee that he will take the preferred action, whatever the state is. 
    This outcome occurs due to the extreme flexibility available to the receiver.
	
\subsubsection{Example: Receiver can only pick one of the phase-II experiment from a finite set} 
This example discusses the receiver's optimal experiment selection if one of the phase-II experiments is already fixed (by other external means) and he is only allowed to pick the second experiment from a given finite set of experiments. Without loss of generality we assume that the fixed experiment is $E_A$ where the receiver knows $(q_{A1},q_{A2})$, and he picks experiment $E_B$ from a finite set $\mathbf{E_B}$, and also knows that the future prior will be in the range $[a,b]$.
%To simplify the discussion, hereafter, we assume that the fixed experiment is $E_A$ where the receiver knows $(q_{A1},q_{A2})$. In this example, the receiver can pick the experiment $E_B$ from a finite set $\mathbf{E_B}$, and she also knows that the future prior will be in the range $[a,b]$. 

To make the result more general, we rule out the second assumption in Claim \ref{clm_asp}, i.e., we do not assume that  experiment $E_A$ is more (Blackwell) informative than the experiment $E_B$ when the true state is $\theta_1$. However, we still assume that the probability of passing a phase-II trial when the true state is $\theta_1$ is greater than or equal to the probability of passing a phase-II trial when the true state is $\theta_2$, i.e., $q_{A1}\geq q_{A2}$ and $q_{B1}\geq q_{B2}$.
    
    When the receiver uses the maximin strategy in knowing the prior region $[a,b]$ under the utility function $U_r(\phi_i,\theta_i)=\mathbf{1}_{\{i=j\}}$, the receiver's objective is to find the experiment $E_B\in \mathbf{E_B}$ that minimizes his maximum probability of taking the wrong action in the prior region $[a,b]$. For example, given $E_A=(1,0)$, $\mathbb{E_{B}}=\{E_{B},E_{\hat{B}}\}$ with $q_{B1}=q_{\hat{B}1}$ and $q_{B2}\geq q_{\hat{B}2}$ and $[a,b]=[0,\frac{q_{B2}}{q_{B1}+q_{B2}}]$, the receiver will choose use experiments $(E_A,E_{\hat{B}})$ instead of $(E_A,E_B)$. If the receiver chooses $(E_A,E_B)$, he will guess incorrectly more often for every prior $p\in [0,\frac{q_{B2}}{q_{B1}+q_{B2}}]$ than when using experiment $(E_A,E_{\hat{B}})$. When the set of available experiment $\mathbf{E_B}$ is small, comparing the receiver's maximin expected utility for each pair of $(E_A,E_B^i),~E_B^i\in \mathbf{E_B}$ in a given prior region is a viable approach. However, when $\mathbf{E_B}$ is large, an approach that efficiently searches through the available experiments $(E_A,E_B^i),~E_B^i\in \mathbf{E_B}$ is required. A preliminary result here provides a partial order of experiments in terms of the receiver's utility. To help in formulating the partial order of experiments, we define a strong notion of inferiority of experiments.

\begin{dfn} \label{dfn:inferior}
An experiment $E_X$ is inferior to an experiment $E_Y$ if the receiver's expected utility of choosing $(E_A, E_Y)$ is higher than the expected utility of choosing $(E_A, E_X)$ for all priors in the specified region and for any given experiment $E_A$.
\end{dfn}
Given the above definition of inferiority, a partial ordered set of $\mathbf{E_B}$ can be built using Lemma \ref{lem:inferior}.
\begin{lem} \label{lem:inferior}
Given two experiments $E_X,E_Y$, $E_X$ is inferior to $E_Y$ if one of the following two conditions is satisfied:
 \begin{align*}
     &(1)~q_{Y1} \leq \frac{2-q_{Y2}}{3-2q_{Y2}} \text{~and~} \max \{2q_{X1}-1, \frac{1-q_{X1}}{1-q_{X2}}\}< \frac{1-q_{Y1}}{1-q_{Y2}}, \\
     &(2)~q_{Y1} > \frac{2-q_{Y2}}{3-2q_{Y2}},~~ q_{X_1}<q_{Y1},\text{~and~} \frac{1-q_{X1}}{1-q_{X2}}<\frac{1-q_{Y_1}}{1-q_{Y2}}.
 \end{align*}
\end{lem}

Lemma~\ref{lem:inferior} can help the receiver to reduce the search of optimal experiments from a large set of experiment candidates, especially when the available experiments is not a countable set. An example in Appendix \ref{appendix:usagelem7} demonstrates how Lemma~\ref{lem:inferior} reduces the set of searching the experiments.


\section{Conclusion}
This work studies Bayesian persuasion problems in multi-phase trials with determined experiments, and highlights the significant difference between single-phase and multi-phase trials: conducted experiments can be correlated in multi-phase trials, and determined experiments can constrain the sender's signalling strategy. When the experiments have binary outcomes, we explicitly analyze the two-phase trial and propose a dynamic programming approach to solve multi-phase trials using backward iteration. We also discuss extensions that study non-binary outcome experiments and analyze scenarios where the determined experiments can be designed by the receiver. 

==> Z_Proof.tex <==
%\newpage
\section{Appendix: Proofs}
\subsection{Proof of Lemma \ref{lem:screening}}
Let's derive the optimal signaling strategy in each scheme and the participants expected utility to validate this claim. First, under different prior regions, the sender's optimal\footnote{to maximize the probability that the receiver will take action $\phi_1$} strategy in a single-phase trial is  to commit to the following signaling strategy:
\begin{table}[h]
\begin{tabular}{|c|c|c|}
\hline
$p\leq \frac{1}{2}$ & $\theta_1$ & $\theta_2$ \\ \hline
$\omega_1$ & p & p \\ \hline
$\omega_2$ & 0 & 1-2p \\ \hline
\end{tabular}
\quad
\begin{tabular}{|c|c|c|}
\hline
$p> \frac{1}{2}$ & $\theta_1$ & $\theta_2$ \\ \hline
$\omega_1$ & p & 1-p \\ \hline
$\omega_2$ & 0 & 0 \\ \hline
\end{tabular}
\end{table}
Given the above signaling strategy, the sender and receiver's expected utility can be calculated in the following table:
\begin{table}[h]
\caption{Table: Sender and Receiver's expected utility in single-phase trials}
\begin{tabular}{|c|c|c|}  
\hline
 & $E[U_s(\phi,\theta)]$ & $E[U_r(\phi,\theta)]$ \\ \hline
$p\leq \frac{1}{2}$ & 2p & 1-p \\ \hline
$p>\frac{1}{2}$ & 1 & p \\ \hline
\end{tabular} \label{tab:1}
\end{table}

In a two-phase trial with a trivial experiment in phase II, we want to solve the sender's optimal signaling strategy. Without loss of generality, let's assume that the trivial experiment is the experiment $E_A$, $q_{A1}=q_{A2}$, and another experiment $E_B$ has $q_{B1}>q_{B2}$. Given these two experiments, the sender's optimal signaling strategy can be derived via solving the following optimization problem:
\begin{align*}
    &\max_{p_1,p_2} P(\omega_A)\mathbf{1}_{\{P(\theta_1|\omega_A)\geq\frac{1}{2}\}}+P(\omega_{BP})\mathbf{1}_{\{P(\theta_1|\omega_{BP})\geq\frac{1}{2}\}}+P(\omega_{BF})\mathbf{1}_{\{P(\theta_1|\omega_{BF})\geq\frac{1}{2}\}} \nonumber \\
    \text{subject~to~}& P(\omega_A)=pp_1+(1-p)p_2 \nonumber\\
     & P(\omega_{BP})=p(1-p_1)q_{B1}+(1-p)(1-p_2)q_{B2} \nonumber\\
     & P(\omega_{BF})=p(1-p_1)(1-q_{B1})+(1-p)(1-p_2)(1-q_{B2}) \nonumber\\
     &P(\theta_1|\omega_A)=\frac{pp_1}{pp_1+(1-p)p_2} \nonumber\\
     & P(\theta_1|\omega_{BP})=\frac{p(1-p_1)q_{B1}}{p(1-p_1)q_{B1}+(1-p)(1-p_2)q_{B2}} \nonumber\\
     & P(\theta_1|\omega_{BF})=\frac{p(1-p_1)(1-q_{B1})}{p(1-p_1)(1-q_{B1})+(1-p)(1-p_2)(1-q_{B2})} \nonumber
\end{align*}

After solving this optimization problem, we can derive the sender and receiver's expected utility in Table \ref{tab:2}:
\begin{table}[ht]
\caption{Sender and Receiver's expected utility under a trivial experiment}
\begin{tabular}{|c|c|c|}  
\hline
 & $E[U_s(\phi,\theta)]$ & $E[U_r(\phi,\theta)]$ \\ \hline
$p\leq \frac{1}{2}$ & 2p & 1-p \\ \hline
$p>\frac{1}{2}$ & 1 & p \\ \hline
\end{tabular} \label{tab:2}
\end{table}

Note that when $q_{B1}=1$, the sender may have multiple optimal signaling strategies when the prior $p$ is low. However, no matter which strategy the sender chooses, the sender and the receiver's expected utilities are the same. 

After checking Table \ref{tab:1} and Table \ref{tab:2}, we validate these two schemes will provide the sender and the receiver the same expected utility under optimal signaling strategies.

% \subsection{Proof of Claim \ref{clm_asp}}
% For the first assumption, if $q_{X1}<q_{X2}$, we can switch the name of outcome "Pass experiment X" and "Pass experiment X." In other words, for such revealed signals $\omega_{XP}$, $\omega_{XF}$, we can replace by signals $\omega'_{XP}$, $\omega'_{XF}$ such that $\omega'_{XP}=\omega_{XF}$ and $\omega'_{XF}=\omega_{XP}$.

% For the second assumption, if $q_{A1}<q_{B1}$, then we can rename the experiments in the second trial. In other words, we can rename experiment $E_A$ to $E_{B'}$ and rename $E_B$ to $E_{A'}$. to make $q_{A'1}\geq q_{B'1}$.

\subsection{Proof of Lemma \ref{lem:tightness}}
We prove this lemma by verifying each strategy's statement, which maximizes the sender's expected utility in each set of strategies, respectively. First, let's recall the IC requirement for each partial strategies listed in Section \ref{sec:IC_in_phase2}.

\begin{table}[h]
\begin{tabular}{|c|l|c|l|}
\hline
 Partial strategy& IC requirement &  Partial strategy& IC requirement\\ \hline
$\alpha_A$ & $p_1\geq \frac{1-p}{p}\frac{q_{A2}}{q_{A1}}p_2$ &
$\alpha_B$ &  $1-p_1\geq \frac{1-p}{p}\frac{q_{B2}}{q_{B1}}(1-p_2)$ \\ \hline
$\beta_A$ & $p_1\geq \frac{1-p}{p}\frac{1-q_{A2}}{1-q_{A1}}p_2$ &
$\beta_B$ &  $1-p_1\geq \frac{1-p}{p}\frac{1-q_{B2}}{1-q_{B1}}(1-p_2)$ \\ \hline
$\gamma_A$ &  
$p_1\leq \frac{1-p}{p}\frac{q_{A2}}{q_{A1}}p_2$&
$\gamma_B$ & 
$1-p_1\leq \frac{1-p}{p}\frac{q_{B2}}{q_{B1}}(1-p_2)$
\\ \hline
\end{tabular}
\end{table}

\begin{enumerate}
    \item \textbf{When $S\in (\alpha_A,\gamma_B)$ or $S\in (\gamma_A,\alpha_B)$}  \\
    Suppose $S$ is a $(\alpha_A,\gamma_B)$ type strategy, the sender's expected utility under $S$ is $pp_1q_{A1}+(1-p)p_2q_{A2}$. Given the definition of persuasion ratio, $pp_1q_{A1}+(1-p)p_2q_{A2}$ is maximized when $p_1=1,p_2=\frac{pp_1}{1-p}\frac{q_{A1}}{q_{A2}}$ or $p_1=1,p_2=1$. Hence, in the former scenario where $p_2=\frac{pp_1}{1-p}\frac{q_{A1}}{q_{A2}}$, IC requirement of $\alpha_A$ is tight in $S$. In the later scenario, the sender sends signal $\omega_A$ with probability one because the prior is larger enough to make the posterior belief of $\theta_1$ conditional on $\omega_{AP}$ to be $\geq \frac{1}{2}$. Hence, the lemma holds when $S$ is a $(\alpha_A,\gamma_B)$ type strategy. 

    Similarly, if $S$ is a $(\gamma_A,\alpha_B)$ type strategy, the sender's expected utility is $p(1-p_1)q_{B1}+(1-p)(1-p_2)q_{B2}$. When sender's expected utility is maximized at $S$, the parameter of $(p_1,p_2)$ is either $p_1=0, p_2=1-\frac{pq_{B1}}{(1-p)q_{B2}}$ or $p_1=0, p_2=0$. The IC requirement of $\alpha_B$ is tight in the former case and $\mathbb{P}(\omega_2)=1$ in the later case. Thus, the lemma holds when $S$ is a $(\alpha_B,\gamma_A)$ type strategy. 
\item \textbf{When $S\in (\beta_A,\gamma_B)$ or $S\in (\gamma_A,\beta_B)$}  \\ 
Suppose $S$ is a $(\beta_A,\gamma_B)$ type strategy, the sender's expected utility is $pp_1+(1-p)p_2$. The strategy $S\in (\gamma_A,\beta_B)$ that maximizes the sender's utility is at $p_1=1, p_2=\frac{p(1-q_{A1})}{(1-p)(1-q_{A2})}$ when $p\leq \frac{1-q{A2}}{2-q_{A2}-q_{A1}}$ or at $p_1=p_2=1$ when $p> \frac{1-q{A2}}{2-q_{A2}-q_{A1}}$. In the former case, the IC requirement of $\beta_A$ is tight. In the later case, the sender will send signal $\omega_1$ with probability 1. Hence, the lemma holds when $S$ is a $(\beta_A,\gamma_B)$ type strategy.
\item \textbf{When $S\in (\alpha_A,\beta_B)$ or $S\in (\beta_A,\alpha_B)$}  \\
 Suppose $S$ is a $(\alpha_A,\beta_B)$ type strategy, the sender's expected utility is
 \begin{align*}
     &pp_1q_{A1}+p(1-p_1)+(1-p)p_2q_{A2}+(1-p)(1-p_2))\\
     =&1-p_1p(1-q_{A1})-p_2(1-p)(1-q_{A2})
 \end{align*}
 when the inequality of IC requirements $\frac{1-p}{p}\frac{q_{A2}}{q_{A1}}p_2\leq p_1\leq \frac{1-p}{p}\frac{1-q_{B2}}{1-q_{B1}}p_2+(1-\frac{1-p}{p}\frac{1-q_{B2}}{1-q_{B1}})$ is satisfied.
 Now, let's discuss the strategy $S$ under different prior region.
 \begin{enumerate}
     \item When $p<\frac{q_{A2}}{q_{A1}+q_{A2}}$, the IC inequality will never be satisfied. Hence, there is no incentive compatible strategy in the set of strategy $S\in (\alpha_A,\beta_B)$ in this region.
     \item When $\frac{q_{A2}}{q_{A1}+q_{A2}} \leq p \leq \frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$, the sender's expected utility is maximized when both inequalities of IC requirements are tight, i.e., \begin{align*}
         (p_1,p_2)=\Bigg(\tfrac{1-\tfrac{1-p}{p}\tfrac{1-q_{B2}}{1-q_{B1}}}{1-\tfrac{q_{A1}}{q_{A2}}\tfrac{1-q_{B2}}{1-q_{B1}}},\tfrac{\tfrac{p}{1-p}-\tfrac{1-q_{B2}}{1-q_{B1}}}{\tfrac{q_{A2}}{q_{A1}}-\tfrac{1-q_{B2}}{1-q_{B1}}}\Bigg).
     \end{align*}
     \item When $p> \frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$, the sender's expected utility is maximized when $p_1=p_2=0$. In other words, the sender will send signal $\omega_2$ with probability 1.
 \end{enumerate}
 After analyzing prior regions (a), (b), and (c), we verify the lemma holds when $S$ is a $(\alpha_A,\beta_B)$ type strategy. 
 
    Similarly, we can use the same approach to verify when $S$ is a $(\beta_A,\alpha_B)$ type strategy.
    
    Suppose $S$ is a $(\beta_A,\alpha_B)$ type strategy, the sender's expected utility is
 \begin{align*}
     &pp_1+(1-p)p_2+p(1-p_1)q_{B1}+(1-p)(1-p_2)q_{B2}\\
     =&1-(1-p_1)p(1-q_{B1})-(1-p_2)(1-p)(1-q_{B2})
 \end{align*}
 when the inequality of IC requirements $\frac{1-p}{p}\frac{1-q_{A2}}{1-q_{A1}}p_2\leq p_1\leq \frac{1-p}{p}\frac{q_{B2}}{q_{B1}}p_2+(1-\frac{1-p}{p}\frac{q_{B2}}{q_{B1}})$ is satisfied.
 Now, let's discuss where the strategy $S$ at under different prior region.
 \begin{enumerate}
     \item When $p<\frac{q_{B2}}{q_{B1}+q_{B2}}$, the IC inequality will never be satisfied. Hence, there is no incentive compatible strategy in the set of strategy $S\in (\alpha_A,\beta_B)$ in this region.
     \item When $\frac{q_{B2}}{q_{B1}+q_{B2}} \leq p \leq \frac{1-p}{p}\frac{q_{A2}}{q_{A1}}(1-p_2)$, the sender's expected utility is maximized when both inequalities of IC requirements are tight, i.e., \begin{align*}
         (p_1,p_2)=\Bigg(\tfrac{1-\tfrac{1-p}{p}\tfrac{q_{B2}}{q_{B1}}}{1-\tfrac{1-q_{A1}}{1-q_{A2}}\tfrac{q_{B2}}{q_{B1}}},\tfrac{\tfrac{p}{1-p}-\tfrac{q_{B2}}{q_{B1}}}{\tfrac{1-q_{A2}}{1-q_{A1}}-\tfrac{q_{B2}}{q_{B1}}}\Bigg).
     \end{align*}
     \item When $p> \frac{1-q_{A2}}{2-q_{A1}-q_{A2}}$, the sender's expected utility is maximized when $p_1=p_2=1$. In other words, the sender will send signal $\omega_1$ with probability 1.
 \end{enumerate}
 After analyzing prior regions (a), (b), and (c), we verify the lemma holds when $S$ is a $(\beta_A,\alpha_B)$ type strategy.
 
\item \textbf{When $S\in (\alpha_A,\alpha_B)$}\\
Suppose $S$ is a $(\alpha_A,\alpha_B)$ type strategy, the sender's expected utility is
 \begin{align*}
     &pp_1q_{A1}+p(1-p_1)q_{B1}+(1-p)p_2q_{A2}+(1-p)(1-p_2))q_{B2}
 \end{align*}
 when the inequality of IC requirements $\frac{1-p}{p}\frac{q_{A2}}{q_{A1}}p_2\leq p_1\leq \frac{1-p}{p}\frac{q_{B2}}{q_{B1}}p_2+(1-\frac{1-p}{p}\frac{q_{B2}}{q_{B1}})$ is satisfied.
 Now, let's discuss the strategy $S$ under different prior region.
 \begin{enumerate}
     \item When $p<\min\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$, the IC inequality will never be satisfied. Hence, there is no incentive compatible strategy in the set of strategy $S\in (\alpha_A,\alpha_B)$ in this region.
     \item When $\min\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\} \leq p \leq \max\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$, the sender's expected utility is maximized when both inequalities of IC requirements are tight, i.e., \begin{align*}
         (p_1,p_2)=\Bigg(\tfrac{1-\tfrac{1-p}{p}\tfrac{q_{B2}}{q_{B1}}}{1-\tfrac{q_{A1}}{q_{A2}}\tfrac{q_{B2}}{q_{B1}}},\tfrac{\tfrac{p}{1-p}-\tfrac{q_{B2}}{q_{B1}}}{\tfrac{q_{A2}}{q_{A1}}-\tfrac{q_{B2}}{q_{B1}}}\Bigg).
     \end{align*}
     \item When $p> \max\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$, the sender's expected utility is maximized when exactly one IC requirement $\alpha_A$ or $\alpha_B$ is tight. \\(For readers curious about which requirement will be tight, the requirement $\alpha_A$ is tight when $p+(1-p)(2q_{A1}-1)\tfrac{q_{A2}}{q_{A1}}+2pq_{B1}-(1-\tfrac{1-p}{p}\tfrac{q_{B2}}{q_{B1}})p(1-2q_{B1})\geq 0$, otherwise, $\alpha_B$ is tight.)
 \end{enumerate}
 After analyzing prior regions (a), (b), and (c), we verify the lemma holds when $S$ is a $(\alpha_A,\beta_B)$ type strategy. 

\item \textbf{When $S\in (\beta_A,\beta_B)$}\\
Suppose $S$ is a $(\beta_A,\beta_B)$ type strategy, the sender's expected utility is 1. However, the IC inequalities of this strategy can be satisfied only if the prior $p\geq \max \big\{\frac{1-q_{A2}}{2-q_{A1}-q_{A2}}, \frac{1-q_{B2}}{2-q_{B1}-q_{B2}}\big\}$.

When $p<\min\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$, the IC inequality will never be satisfied. Hence, there is no incentive compatible strategy in the set of strategy $S\in (\alpha_A,\alpha_B)$ in this region.


\end{enumerate}

\subsection{Proof of Lemma \ref{lem:conveshull}}
First, since $(\gamma_A,\gamma_B)$ strategy has a persuasion ratio $0$ when $\mathcal{S}_{\gamma_A,\gamma_B}(p)\neq \emptyset$, the statement in the lemma for each set of strategies: $(\alpha_A,\gamma_B)$, $(\beta_A,\gamma_B)$, $(\gamma_A,\alpha_B)$, and $(\gamma_A,\beta_B)$ is true. Hence, we only need to verify this lemma for the following four sets of strategies: (1) $(\alpha_A,\alpha_B)$, (2) $(\alpha_A,\beta_B)$, (3) $(\beta_A,\alpha_B)$, and (4) $(\beta_A,\beta_B)$.

Let's start with the type of strategies $(\alpha_A,\alpha_B)$.\\
        The IC requirements of this type of strategy can be satisfied when $p\geq \min\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$, i.e., $\mathcal{S}_{\alpha_A,\alpha_B}(p)\neq \emptyset$ when $p\geq \min\big\{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\big\}$. When the IC requirements are satisfied, the sender's expected utility under a strategy $\{(\alpha_A,\alpha_B), p_1, p_2\}$ is
         \begin{align*}
            &E[U_s(p|(\alpha_A,\alpha_B), p_1, p_2)]=pp_1q_{A1}+p(1-p_1)q_{B1}+(1-p)p_2q_{A2}+(1-p)(1-p_2))q_{B2}.
        \end{align*}
        
        Besides, the sender's expected utility under strategies $\{(\alpha_A,\gamma_B), p_1, p_2\}$ and $\{(\gamma_A,\alpha_B), p_1, p_2\}$ are the following:
        \begin{align*}
            &E[U_s(p|(\alpha_A,\gamma_B), p_1, p_2)]=pp_1q_{A1}+(1-p)p_2q_{A2},\\
            &E[U_s(p|(\gamma_A,\alpha_B), p_1, p_2)]=p(1-p_1)q_{B1}+(1-p)(1-p_2))q_{B2}.
        \end{align*}
        
        Given the result in Lemma \ref{lem:tightness}, we know that $E[U_s(p|(\alpha_A,\gamma_B), p_1, p_2)]$ can be represented by a scaled optimized signaling strategy under another prior $u$ such that $xu=pp_1$ and $E[U_s(p|(\alpha_A,\gamma_B), p_1, p_2)]= xuPR(\alpha,\gamma,u)$. (Because an optimized strategy $\arg\max_{S\in (\alpha_A,\gamma_B, p_1',p_2')} E[U_r(S,p')]$ must have $p_1'=1$ in the optimized $S$.) 
        Similarly, we can represent $E[U_s(p|(\gamma_A,\alpha_B), p_1, p_2)]$ as a scaled optimized signaling strategy under another prior $v$ such that $(1-x)v=p(1-p_1)$ and $E[U_s(p|(\gamma_A,\alpha_B), p_1, p_2)]= (1-x)vPR(\gamma,\alpha,u)$. Hence,
        \begin{align*}
        &\max_{p_1,p_2} E[U_s(p|(\alpha_A,\alpha_B), p_1, p_2)]\\
        =&(\max_{p_1,p_2} pp_1q_{A1}+p(1-p_1)q_{B1}+(1-p)p_2q_{A2}+(1-p)(1-p_2))q_{B2})\\
        =&\max_{p_1,p_2} \big(E[U_s(p|(\alpha_A,\gamma_B), p_1, p_2)]+E[U_s(p|(\gamma_A,\alpha_B), p_1, p_2)]\big)\\
        =&\max_{x,u,v} xuPR((\alpha_A,\gamma_B),u)+ (1-x)vPR((\gamma_A,\alpha_B),v) 
        {~s.t.~} xu+(1-x)v=p
        \end{align*}
    
        Now, let $y=\frac{xu}{p}$, we can represent the persuasion ratio curve of $(\alpha_A,\alpha_B)$ strategy to be the following:
  
        \begin{align*}
        PR((\alpha_A,\alpha_B),p)=&\max_{p_1,p_2} E[U_s(p|(\alpha_A,\alpha_B), p_1, p_2)]/p\\
        =&\max_{x,u,v} \frac{xu}{p}PR((\alpha_A,\gamma_B),u)+ \frac{(1-x)v}{p}PR((\gamma_A,\alpha_B),v) 
        {~s.t.~} xu+(1-x)v=p \\
        =&\max_{y,u,v} \{yPR((\alpha_A,\gamma_B),u)+ (1-y)PR((\gamma_A,\alpha_B),v) \big| yu+(1-y)v=p~~y\in [0,1]\}
        \end{align*}      
        
Using the same approach, we can represent the maximum expected utility of the set of strategy $(\alpha_A,\beta_B)$,  $(\beta_A,\alpha_B)$, $(\beta_A,\beta_B)$ in the form of a maximum convex combination of two persuasion ratio curves by using the corresponding two of four utility functions listed below:
        \begin{align*}
        &E[U_s(p|(\alpha_A,\gamma_B), p_1, p_2)]=pp_1q_{A1}+(1-p)p_2q_{A2},\\
            &E[U_s(p|(\gamma_A,\alpha_B), p_1, p_2)]=p(1-p_1)q_{B1}+(1-p)(1-p_2))q_{B2},\\
            &E[U_s(p|(\beta_A,\gamma_B), p_1, p_2)]=pp_1+(1-p)p_2,\\
            &E[U_s(p|(\gamma_A,\beta_B), p_1, p_2)]=p(1-p_1)+(1-p)(1-p_2).
        \end{align*}

\subsection{Proof of Lemma \ref{lem:optbny}}
     Given persuasion ratio curves of all types of strategies, the sender, in order to maximize her expected utility, will choose the type of strategies with the highest persuasion ratio. (Because the persuasion ratio indicates a ``normalized'' utility with respect to the prior.) When we plot the persuasion ratio the sender chooses for every prior, the optimal persuasion ratio curve is the upper envelope of the different types of strategies' persuasion ratio curves. We want to explain why the persuasion ratio that the sender chooses to maximize her expected utility must correspond to an incentive-compatible strategy. According to Definition \ref{prcurve}, every non-zero point on the persuasion ratio curve of a given type of strategy corresponds to at least one incentive-compatible strategy. Hence, we need to show that at every prior $p\in (0,1)$, there must exist a type of strategy with a persuasion ratio $>0$.
     \begin{enumerate}
         \item When $0<p<\frac{q_{A2}}{q_{A1}+q_{A2}}$, the type of strategy $(\alpha_A,\gamma_B)$ has an incentive compatible strategies with persuasion ratio $2q_{A1}$.
         \item When $\frac{q_{A2}}{q_{A1}+q_{A2}}\leq p<\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$, the type of strategy $(\alpha_A,\beta_B)$ has an inventive compatible strategy with persuasion ratio $\geq \min\{2q_{A1}, 1+\frac{1-q_{B1}}{1-q_{B2}}\}$.
         \item When $\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}\leq p<1$, the type of strategy $(\gamma_A,\beta_B)$ has an inventive compatible strategy with persuasion ratio $\frac{1}{p}$.
     \end{enumerate}
    Given the fact (1), (2), and (3), the value of the optimal persuasion ratio curve is non-zero for every $p\in (0,1)$. Hence, the optimal signaling strategy is the strategy that reaches the frontier of the persuasion ratio curve.

\subsection{Proof of Lemma \ref{lem:nphasebp}}
We want to prove this lemma by constructing an optimal signaling strategy in the pruned model, which has the same expected utility as the single-phase Bayesian persuasion problem. 

Let's assume there is an $N$-phase model $M$ which pruned model $Prun(M)$ satisfies the above two conditions stated in Lemma \ref{lem:nphasebp} and a prior $p<\frac{1}{2}$. We want to construct a signaling strategy that gives the sender the expected utility is equal to $2p$ (which is the same as the single-phase Bayesian persuasion.

First, for each non-trivial experiment $E_X$, design its preceding sender-designed experiment such that $\mathbb{P}(\theta_1|\omega_X)=\mathbb{P}(\theta_2|\omega_X)=0$. In other words, we assign probability $0$ to the experiment $E_X$. After the above process, if there exists some sender-designed experiments, design these experiments to be (arbitrary chosen) trivial experiment with $p_1=p_2$.

Now, let $\mathbb{E_F}$ be the set of sender-designed experiments such that for every $E_f\in \mathbb{E_F}$, there is no sender-designed experiment between this experiment $E_f$ and the experiment at root $E_o$. In other words, $\mathbb{E_F}$ is the set of first-visited sender-designed experiments starting from the root. For every experiment $E_f=(p_1,p_2)\in \mathbb{E_F}$ with succeeding experiment $E_l,E_r$ let $(p_1,p_2)=(1,\frac{p}{1-p})$ if the experiment lower succeeding experiment $E_r$ is a non-trivial experiment, otherwise let $(p_1,p_2)=(0,1-\frac{p}{1-p})$. Hence, the posterior belief $\mathbb{P}(\theta_1|omega)$ in this pruned model $\mathbb{M}$ is either $0$ or $\frac{1}{2}$. Since the whole signal distribution must respect the prior, the sender will have an expected utility $2p$ under this construction, which is the same as the classical Bayesian persuasion in single-phase model.

\subsection{Proof of Lemma \ref{lem:receiverexp}}
Given the receiver's utility function defined in this work, i.e., $U_r(\phi_i,\theta_j)=\mathbf{1}_{\{i=j\}}$, the receiver's utility is maximized when the sender commits to a truth-telling signaling strategy. Given the phase-II experiments $E_A=(1,0)$ and $E_B=(1,0)$ stated in the lemma, the posterior belief in each possible outcome $\mathbb{P}(\theta_1|\omega_{AP}),\mathbb{P}(\theta_1|\omega_{AF}),\mathbb{P}(\theta_1|\omega_{BP}),\mathbb{P}(\theta_1|\omega_{BF}) \in \{0,1\}$ for any $(p_1,p_2)\in [0,1]^2$ where the sender choose in phase-I experiment. In other words, the receiver knows exactly the true state is for every possible realized outcome $\omega \in \{\omega_{AP},\omega_{AF},\omega_{BP},\omega_{BF}\}$. Hence, for any prior $p$, the receiver will have an utility $E[U_r(\omega,p)]=1$, which is the maximum utility the receiver can have under the given utility function.

\subsection{Proof of Lemma \ref{lem:inferior}}
%\textcolor{red}{This proof needs to be rewritten to satisfy updated statements in the Lemma. The proof is basically a list of comparisons of the receiver's expected utility between two experiments under each possible partial strategy combination.} 

First, let's consider the case when $q_{Y1} \leq \frac{2-q_{Y2}}{3-2q_{Y2}}$. 
\begin{enumerate}
    \item Suppose a given experiment $E_A$ has $\max\{2q_{A1}-1,\frac{1-q_{A2}}{1-q_{A1}}\}\leq \frac{1-q_{Y2}}{1-q_{Y1}}$, the optimal signaling strategy of $(E_A,E_Y)$ when $P(\phi_1|\Pi)<1$ is $(\gamma_A,\beta_Y)$. Hence, if $\max \{2q_{X1}-1, \frac{1-q_{X1}}{1-q_{X2}}\}< \frac{1-q_{Y1}}{1-q_{Y2}}$, the persuasion ratio curve of any type of IC strategy $(c_A,d_X)$ with $c,d\in \{\alpha,\beta,\gamma\}$ has a persuasion ratio $\leq 1+\frac{1-q_{Y2}}{1-q_{Y1}}$, for every possible prior. Hence, the lemma holds in this case.
    \item Suppose a given experiment $E_A$ has $\max\{2q_{A1}-1,\frac{1-q_{A2}}{1-q_{A1}}\}> \frac{1-q_{Y2}}{1-q_{Y1}}$ and $2q_{A1}>1+\frac{1-q_{A2}}{1-q_{A1}}$, the optimal signaling strategy of $(E_A,E_B), B\in \{X,Y\}$ when $P(\phi_1|\Pi)<1$ is $(\alpha_A,\gamma_B)$, $(\alpha_A,\beta_B)$, or $(\beta_A,\gamma_B)$ depending on the prior region. Given $\max \{2q_{X1}-1, \frac{1-q_{X1}}{1-q_{X2}}\}< \frac{1-q_{Y1}}{1-q_{Y2}}$, the persuasion ratio of $(\alpha_A,\beta_Y)$ is higher than $(\alpha_A,\beta_X)$ for every prior $p$ such that $(\alpha_A,\beta_Y)$, $(\alpha_A,\beta_X)$ have IC strategies. Hence, the lemma holds in this case.
    \item Suppose a given experiment $E_A$ has $\max\{2q_{A1}-1,\frac{1-q_{A2}}{1-q_{A1}}\}> \frac{1-q_{Y2}}{1-q_{Y1}}$ and $2q_{A1}<1+\frac{1-q_{A2}}{1-q_{A1}}$, the optimal signaling strategy of $(E_A,E_B), B\in \{X,Y\}$ when $P(\phi_1|\Pi)<1$ is always a $(\beta_A,\gamma_B)$ type strategy. Hence, the statement of lemma holds in this case. 
\end{enumerate}
After considering all scenarios under $q_{Y1} \leq \frac{2-q_{Y2}}{3-2q_{Y2}}$, we know that if $\max \{2q_{X1}-1, \frac{1-q_{X1}}{1-q_{X2}}\}< \frac{1-q_{Y1}}{1-q_{Y2}}$, then $E_X$ is inferior to $E_Y$.

Now, let's consider the case when $q_{Y1} > \frac{2-q_{Y2}}{3-2q_{Y2}}$. $E_X$ is inferior to $E_Y$ requires for every prior $p$, the inequality of optimal persuasion ratio $PR^*_{E_A,E_x}(p) \leq PR^*_{E_A,E_x}(p)$ holds. Since the experiment $E_A$ can be arbitrarily given, $E_X$ is inferior to $E_Y$ requires the persuasion ratio curve of different type of strategies under $(E_A,E_x)$ is always below the persuasion ratio curve of different type of strategies under $(E_A,E_Y)$. Using the partial strategy analysis in Section \ref{sec:IC_in_phase2}, the above condition requires every class of partial strategies $c_B$, $c\in \{\alpha,\beta\},~B\in \{X,Y\}$, using experiment $E_X$ is always inefficient than using experiment $E_X$. That is to say, $2q_{X_1}<2q_{Y1}$ and $1+\frac{1-q_{X1}}{1-q_{X2}}<1+\frac{1-q_{Y_1}}{1-q_{Y2}}$ according to the persuasion potential of $E_X$ and $E_Y$. Hence, when $q_{Y1} > \frac{2-q_{Y2}}{3-2q_{Y2}}$, the condition derived from persuasion potential guaranteeing that $E_X$ is inferior to $E_Y$ satisfy the second condition stated in the lemma.

% Similar to the result in Lemma \ref{lem:receiverexp}, the receiver's expected utility is maximized while choosing $E_X=(1,0)$. However, unlike the case where the receiver can choose both experiments, there are plenty of experiments $E_X'$ which gives the receiver the same maximin expected utility as $E_X=(1,0)$ under a given $E_Y$.

% Since the receiver knows the experiment $E_Y=(q_{Y1},q_{Y2})$ and its corresponding persuasion potential $PerP(E_Y)=(2q_{Y1},1+\frac{1-q_{Y1}}{1-q_{Y2}})$, we should analyze the set of $E_X$ giving the receiver a maximin expected utility under different $(q_{Y1},q_{Y2})$ region.

% When $2q_{Y1}\leq 1+\frac{1-q_{Y1}}{1-q_{Y2}}$, we can observe that there is an optimal signaling strategy under $E_X=(1,0),E_Y$ using the type of strategy $(\gamma_X,\beta_Y)$ whatever the prior $p$ is. Given this observation, the set of experiment $E_X\in \mathcal{E}_X$ such that $\mathbb{P}(\omega_X)=0$ under the optimal signaling strategy will give the receiver same (maximin) expected utility. The set of experiments which has a persuasion potential $(2q_{X1}, 1+\frac{1-q_{X1}}{1-q_{X2}})$ such that $\max \{1+2q_{X1}, 1+\frac{1-q_{X1}}{1-q_{X2}}\}< 1+\frac{1-q_{Y1}}{1-q_{Y2}}$ can satisfy the condition $\mathbb{P}(\omega_X)=0$ because the persuasion ratio curve using which will use $\alpha_X$ or $\beta_X$ partial strategies will always be below to the persuasion ratio curve $(\gamma_X,\beta_Y)$. This set of experiments is the condition (1) of inferiority in Definition $\ref{dfn:inferior}$.

% When $2q_{Y1}> 1+\frac{1-q_{Y1}}{1-q_{Y2}}$, the sender's optimal signaling strategy under $E_X=(1,0),E_Y$ uses the type of strategy $(\gamma_X,\alpha_Y)$ in the low prior region $p\leq \frac{q_{Y2}}{q_{Y1}+q_{Y2}}$, $(\beta_X,\alpha_Y)$ in the middle prior region $\frac{q_{Y2}}{q_{Y1}+q_{Y2}}<p<\frac{1-q_{Y2}}{2-q_{Y1}-q_{Y2}}$, and $(\gamma_X,\beta_Y)$ in the high prior region $p\geq \frac{1-q_{Y2}}{2-q_{Y1}-q_{Y2}}$.


\subsection{Proof of Corollary \ref{cor:perppowerful}}
When the prior $p\geq \min \{\frac{1-q_{A2}}{2-q_{A1}-q_{A2}},\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}\}$, the sender has an optimal signaling strategy to persuade the receiver to take action $\phi_1$ with probability one by $(p_A,p_B)=(1,1)$ when $\frac{1-q_{A2}}{2-q_{A1}-q_{A2}}\leq \frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$ or by $(p_A,p_B)=(0,0)$ when $\frac{1-q_{A2}}{2-q_{A1}-q_{A2}}> \frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$. Hence, to prove this lemma, we only need to consider the prior region $p\in [0, \min \{\frac{1-q_{A2}}{2-q_{A1}-q_{A2}},\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}\})$.

First, let's consider $p\in [0, \min \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}]$. When prior falls in this region, four type of strategies: $(\alpha_A,\alpha_B)$, $(\alpha_A,\beta_B)$, $(\beta_A,\alpha_B)$, $(\beta_A,\beta_B)$ cannot satisfy the IC requirements\footnote{See Proof of Lemma \ref{lem:tightness} for details.}. Hence, the optimal signaling strategy can only come from $(\alpha_A,\gamma_B)$, $(\beta_A,\gamma_B)$, $(\gamma_A,\alpha_B)$, $(\gamma_A,\beta_B)$ types of strategies. Given the result of Lemma \ref{lem:tightness}, the IC requirement of $\alpha$ or $\beta$ partial strategy used in the optimal signaling strategy must be tight. This implies the interim belief of $\alpha_X$ strategy must be $\frac{q_{X2}}{q_{X1}+q_{X2}}$ and the interim belief of $\beta_X$ strategy $\frac{1-q_{X2}}{2-q_{X1}-q_{X2}}$ (otherwise the IC requirement is not tight). Under these interim belief, the $\alpha_X,\beta_X$ partial strategy is used in the most efficient manner as described in Section \ref{sec:IC_in_phase2} and the corollary holds here.

Second, let's consider $p\in [\min \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}, \max \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}]$. When the prior falls in this region, the optimal signaling strategy can come from one of the 6 types of strategies\footnote{$(\gamma_A,\alpha_B)$ cannot be an optimal signaling strategy in this region because $q_{A1}\geq q_{B1}$ is assumed in our framework.}: $(\alpha_A,\gamma_B)$, $(\beta_A,\gamma_B)$, $(\gamma_A,\beta_B)$,  $(\alpha_A,\alpha_B)$, $(\alpha_A,\beta_B)$, $(\beta_A,\alpha_B)$. Recall the analysis in the proof of Lemma \ref{lem:tightness}, when a strategy in the type of $(\alpha_A,\beta_B)$, $(\beta_A,\alpha_B)$, or $(\alpha_A,\alpha_B)$ maximizes the sender's expected utility in this prior region, both IC requirements are tight. Besides, when a strategy in the type of $(\beta_A,\gamma_B)$ or $(\gamma_A,\beta_B)$ maximizes the sender's expected utility in this prior region, the IC requirement of $\beta_X$ is tight. Hence, the only possibility for this corollary to fail is when the optimal signaling strategy is a $(\alpha_A,\gamma_B)$ type strategy. Now, we prove that the optimal signaling strategy is never an $(\alpha_A,\gamma_B)$ type strategy in this prior region by comparing the sender's maximum expected utility between $(\alpha_A,\gamma_B)$ and $(\alpha_A,\beta_B)$ type strategies.

Under $(\alpha_A,\gamma_B)$ type strategy, the sender's expected utility is maximized when $(p_1,p_2=1)$. Hence, $U_s((\alpha_A,\gamma_B),p)=pq_{A1}+(1-p)q_{A2}$ in this prior region.

Under $(\alpha_A,\beta_B)$ type strategy, the sender's expected utility is maximized when $\mathbb{P}(\theta_1|E_A)=\frac{q_{A2}}{q_{A1+q_{A2}}}$ and $\mathbb{P}(\theta_1|E_B)=\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}$. Hence, $U_s((\alpha_A,\beta_B),p)=2\frac{\mathbb{P}(\theta_1|E_B)-p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\mathbb{P}(\theta_1|E_A)q_{A1}+(1-\frac{\mathbb{P}(\theta_1|E_B)-p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)})$.

When we look at the sender's maximum expected utility under these two types of strategies, we can notice that $U_s((\alpha_A,\gamma_B),p)=U_s((\alpha_A,\beta_B),p)$ at $p=\frac{q_{A2}}{q_{A1}+q_{A2}}$, which is the minimum prior in this region. When p increases, the marginal utility gain at $(\alpha_A,\gamma_B)$ type strategy is $q_{A1}-q_{A2}$, and the marginal utility gain at $(\alpha_A,\beta_B)$ type strategy is 
\begin{align*}
    \frac{-2}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\mathbb{P}(\theta_1|E_A)q_{A1}+\frac{1}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}=\frac{1-2q_{A1}\mathbb{P}(\theta_1|E_A)}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)})
\end{align*}
Thus, the utility difference $U_s((\alpha_A,\beta_B),p)-U_s((\alpha_A,\gamma_B),p)$ in this prior region is
\begin{align*}
    &p\times \Big(\frac{1-2q_{A1}\mathbb{P}(\theta_1|E_A)}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)})-(q_{A1}-q_{A2})\Big) \\
    =&\frac{p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\times \Big(1-2q_{A1}\mathbb{P}(\theta_1|E_A)-(\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A))(q_{A1}-q_{A2})\Big) \\
    =&\frac{p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\times \Big(1-\mathbb{P}(\theta_1|E_A)(q_{A1}+q_{A2})-\mathbb{P}(\theta_1|E_B)(q_{A1}-q_{A2})\Big) \\
    =&\frac{p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\times \Big(1-q_{A2}-\mathbb{P}(\theta_1|E_B)(q_{A1}-q_{A2})\Big) \\
    =&\frac{p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\times \Big(1-\frac{(1-q_{B2})q_{A1}+(1-q_{B1})q_{A2}}{2-q_{B1}-q_{B2}}\Big) \\
    >&\frac{p}{\mathbb{P}(\theta_1|E_B)-\mathbb{P}(\theta_1|E_A)}\times \Big(1-q_{A1}\Big) \geq 0.
\end{align*}
    Given the calculation above, we know that $(\alpha_A,\gamma_B)$ type strategy will never be an optimal signaling strategy in this prior region. Hence, the corollary holds in this prior region. 

Last, we want to consider $p\in [\max \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}, \min \{\frac{1-q_{A2}}{2-q_{A1}-q_{A2}},\frac{1-q_{B2}}{2-q_{B1}-q_{B2}}\}]$. When prior falls in this region, all except the $(\beta_A,\beta_B)$ strategies can satisfy the IC requirements. Given the tightness analysis in the proof of Lemma \ref{lem:tightness}, the corollary will fail if the optimal signaling strategy comes from type $(\alpha_A,\gamma_B)$, $(\gamma_A,\alpha_B)$, or $(\alpha_A,\alpha_B)$. To rule out $(\alpha_A,\gamma_B)$, $(\gamma_A,\alpha_B)$, we use exactly the same calculation as we did in the prior region $p\in [\min \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}, \max \{\frac{q_{A2}}{q_{A1}+q_{A2}},\frac{q_{B2}}{q_{B1}+q_{B2}}\}]$. Hence, the only interesting case to study is whether $(\alpha_A,\alpha_B)$ type strategy can be an optimal signaling strategy in this prior region.

Suppose $(\alpha_A,\alpha_B)$ type strategy is an optimal signaling strategy in this prior region, at most one $IC$ requirement, which is $\alpha_A$, can be tight. When the IC requirement of $\alpha_A$ is not tight, the strategy is not an optimal signaling strategy since one the sender can increase her expected payoff by increasing $\mathbb{P}(\omega_A)$ and reduce $\mathbb{P}(\omega_A)$ respecting the prior. When the IC requirement of $\alpha_A$ is tight and $(\alpha_A,\beta_B)$ is not an incentive compatible strategy for the receiver, the following modification can further increase the sender's expected utility:
\begin{itemize}
    \item Reduce $\mathbb{P}(\theta_1,\omega_B)$ by $\epsilon$ but increase $\mathbb{P}(\theta_1,\omega_A)$ by $\epsilon$;
    \item Given the above $\epsilon$, reduce $\mathbb{P}(\theta_2,\omega_B)$ by $\frac{1-q_{A1}}{1-q_{A2}}\epsilon$ but increase $\mathbb{P}(\theta_2,\omega_A)$ by $\frac{1-q_{A1}}{1-q_{A2}}\epsilon$.
\end{itemize}
When $(\alpha_A,\beta_B)$ is not an incentive compatible strategy for the receiver, there must exists an $\epsilon>0$ such that the above modification constructs a new incentive compatible strategy. When $\epsilon$ is picked such that $(\alpha_A,\beta_B)$ is an incentive compatible strategy for the receiver, strategy $(\alpha_A,\beta_B)$ gives a higher expected utility than strategy $(\alpha_A,\beta_B)$ under the same parameter of $(p_1,p_2)$. Hence, $(\alpha_A,\alpha_B)$ is never an optimal signaling strategy (in this prior region) and the corollary holds.
\subsection{Proof of Claim \ref{clm_asp}}
Suppose we have a phase-II experiment $E_X,~X\in\{A,B\}$ which violates $q_{X1} \geq q_{X2}$, then we can replace this experiment $E_X$ by another experiment $E_X'$ such that $q_{X'1}=q_{X2}$ and $q_{X'2}=q_{X1}$ to satisfy the assumption. For every interim belief $\Tilde{p}_X$, this operation (of replacement) will not affect the sender's design room of optimal signaling strategies because the posterior belief $\mathbb{P}(\theta_1|\Tilde{p}_X, \omega_XP)=\mathbb{P}(\theta_1|\Tilde{p}_X, \omega_X'F)$ and the posterior belief $\mathbb{P}(\theta_1|\Tilde{p}_X, \omega_XF)=\mathbb{P}(\theta_1|\Tilde{p}_X, \omega_X'P)$. Hence, the first assumption in Claim \ref{clm_asp} can be made without loss of generality.

Suppose we have phase-II experiments $E_A,E_B$ such that $q_{A1}\leq q_{B1}$, then we can replace experiments $E_A,E_B$ by experiments $E_{A'},E_{B'}$ such that $q_{A'1}=q_{B1}$ and $q_{B'1}=q_{A1}$ to satisfy the assumption. This operation (of replacement) will not affect the sender's design room because the posterior belief $\mathbb{P}(\theta_1|\omega_AY)=\mathbb{P}(\theta_1|\omega_B'Y),~Y\in\{P,F\}$ and the posterior belief $\mathbb{P}(\theta_1|\omega_BY)=\mathbb{P}(\theta_1|\omega_A'Y),~Y\in\{P,F\}$. Hence, the second assumption in Claim \ref{clm_asp} can be made without loss of generality.

\subsection{Proof of Claim \ref{clm0}}
Given that $q_{X1}\geq q_{X2}$, let's calculate the posterior of outcome $\omega_{XP}$ and $\omega_{XF}$. Suppose an interior beleif of $\mathbb{P}(\theta_1|\omega_X)=\Tilde{p}$, the posterior belief $\mathbb{P}(\theta_1|\omega_{XP})=\frac{\Tilde{p}q_{X1}}{\Tilde{p}q_{X1}+(1-\Tilde{p})q_{X2}}$ and the posterior belief $\mathbb{P}(\theta_1|\omega_{XF})=\frac{\Tilde{p}(1-q_{X1})}{\Tilde{p}(1-q_{X1})+(1-\Tilde{p})(1-q_{X2})}$.

Given that $q_{X1}\geq q_{X2}$, 
\begin{align*}
    \mathbb{P}(\theta_1|\omega_{XP})&=\frac{\Tilde{p}q_{X1}}{\Tilde{p}q_{X1}+(1-\Tilde{p})q_{X2}}\\
    &>\frac{\Tilde{p}q_{X1}}{\Tilde{p}q_{X1}+(1-\Tilde{p})q_{X1}}=\frac{\Tilde{p}}{\Tilde{p}+(1-\Tilde{p})}=\frac{\Tilde{p}(1-q_{X1})}{\Tilde{p}(1-q_{X1})+(1-\Tilde{p})(1-q_{X1})}\\
    &>\frac{\Tilde{p}(1-q_{X1})}{\Tilde{p}(1-q_{X1})+(1-\Tilde{p})(1-q_{X2})}=\mathbb{P}(\theta_1|\omega_{XF}).
\end{align*}
Hence, taking action $\phi_1$ when $E_X$ fails but taking action $\phi_2$ when $E_X$ passes is not an incentive compatible strategy of the receiver for any interim belief $~\mathbb{P}(\theta_1|E_X)\in [0,1]$.
\subsection{Proof of Claim \ref{clm2}}
Given $PR^*_{L+1,2j-1}(p)$ and $PR^*_{L+1,2j}(p)$, We show that there exists an incentive compatible strategy $S_{L,j,+}$ starting from the experiment $E_{L,j}$ satisfies the following equation: 
    \begin{align} \label{eqn:5}
        PR_{L,j}(S_{L,j,+},p)=\max_{x,u,v\in[0,1],xu+(1-x)v=p}xPR^*_{L+1,2j-1}(u)+(1-x)
        PR^*_{L+1,2j}(v)
    \end{align}

Let's prove it by mathematical induction. When $L=N-2$, Lemma \ref{lem:optbny} tells that every point on an optimal persuasion ratio curve at $N-1$ corresponds to at least one incentive compatible strategy. Hence, a strategy $S_{L,j,+}$ which uses experiment $E_{L,j}=\big(\frac{xu}{p},\frac{x(1-u)}{1-p}\big)$ at phase $L$ and the optimal IC signaling strategies at $E_{L+1,2j-1}$, $E_{L+1,2j}$ satisfying equation (\ref{eqn:5}). The reason is that the role of experiment $E_{L,i}$ is to determining what incentive compatible strategies will be used at phase $L+1$ by influencing the interim belief at phase $L+1$. As long as the strategies taken at phase $L+1$ satisfies the IC requirements, $S_{L,j,+}$ is also an incentive compatible strategy.

Suppose the statement is true at phase $L+1$ and the corresponding optimal signaling strategies are $S_{L+1,2j-1,+}$ and $S_{L+1,2j,+}$, there exists an incentive compatible strategy $S_{L,j,+}$ such that $E_{L,j}=\big(\frac{xu}{p},\frac{x(1-u)}{1-p}\big)$, where $x,u,v$ are parameters corresponding to a maximized (\ref{eqn:5}). Given the interim prior after conducting the experiment $E_{L,j}$, $S_{L,j,+}$ will use the optimal signaling strategy $S_{L+1,2j-1,+}$ and $S_{L+1,2j,+}$ to make equation (\ref{eqn:5}) holds. By doing this, $S_{L+1,2j,+}$ is now an incentive compatible strategy satisfying the statement and the proof is complete here.

\subsection{Proof of Claim \ref{clm:nbnry}}
We present a construction to substitute a given non-binary experiment $E=\{q_{1,1},...,q_{1,n};q_{2,1},...,q_{2,n}\}$ by a sequence of binary outcome experiments.

First, we construct a level $\lceil \log_2n \rceil$ of binary-outcome experiments - $\{E'_{1,1},E'_{2,1},E'_{1,2},...,E'_{\lceil \log_2n \rceil,2^{\lceil \log_2n \rceil}}\}$ - 
that we will use for replacement.
Specifically, let $E_{i,j}$ to be the experiment below:
\begin{align*}
    \Big(\frac{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}}{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}+\sum_{l=2^{i-1}\cdot (j-2)+1}^{2^{i-1}\cdot (j-1) }q_{1,l}},\frac{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{2,k}}{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}+\sum_{l=2^{i-1}\cdot (j-2)+1}^{2^{i-1}\cdot (j-1)} q_{2,l}} \Big)
\end{align*}
when $i$ is even, and

\begin{align*}
    \Big(\frac{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}}{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}+\sum_{l=2^{i-1}\cdot j+1}^{2^{i-1}\cdot (j+1) }q_{1,l}},\frac{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{2,k}}{\sum_{k=2^{i-1}\cdot (j-1)+1}^{2^{i-1}\cdot j}q_{1,k}+\sum_{l=2^{i-1}\cdot j+1}^{2^{i-1}\cdot (j+1)} q_{2,l}} \Big)
\end{align*}
when $i$ is odd.

Since the denominator's sum is $1$ in $E_{1,1}$, and the nominator cancels the denominator in the next level. Hence, when we product from the first level to the last level, the $k^{th}$ outcome should have $(q_{k,1},q_{k,2})$.
 
\section{Appendix: Other related work}~\label{appendix:otherwork}

The topic of a constrained sender has received significant attention in the literature with the constraints arising in a varied manner. The work in \cite{perez:prady:complicating:2012,perez:interim:2014} proves that pooling equilibria result if the receiver either performs a certification or validation process; the results allow for the signals of the sender to be exogenously constrained. There is a large body of work that considers scenarios where the constraints arise either due to communication costs~\cite{gentzkow:kamenica:costly:2014,hedlund:costly:2015,carroni:ferrari:pignataro:quality:2020,nguyen2019bayesian}, capacity limitations~\cite{le2019persuasion}, the sender's signal playing multiple roles~\cite{boleslavsky:kim:bayesian:2018} (e.g. incentivizing a third party to take a payoff-relevant action), or costs to the receiver for acquiring additional information~\cite{matyskova:bayesian:2018}.  These works characterize either the applicability of the concavization approach~\cite{kamenica2011bayesian}, the optimal signaling structure, or the conditions for the optimality of certain signaling structures. There is also a burgeoning literature on constraints on the sender arising from a privately informed receiver~\cite{kolotilin:mylovanov:zapechelnyuk:li:persuasion:2017,guo:shmmaya:interval:2019,doval:skreta:constrained:2018,candogan:reduced:2020,candogan:strack:optimal:2021}. The main contributions here are to characterize the optimal signaling structure with a key aspect being the fact that the sender constructs a different signal for each receiver type. 
